Synthetic Data in Human Analysis: A Survey

Deep neural networks have become prevalent in human analysis, boosting the performance of applications, such as biometric recognition, action recognition, as well as person re-identification. However, the performance of such networks scales with the available training data. In human analysis, the demand for large-scale datasets poses a severe challenge, as data collection is tedious, time-expensive, costly and must comply with data protection laws. Current research investigates the generation of \textit{synthetic data} as an efficient and privacy-ensuring alternative to collecting real data in the field. This survey introduces the basic definitions and methodologies, essential when generating and employing synthetic data for human analysis. We conduct a survey that summarises current state-of-the-art methods and the main benefits of using synthetic data. We also provide an overview of publicly available synthetic datasets and generation models. Finally, we discuss limitations, as well as open research problems in this field. This survey is intended for researchers and practitioners in the field of human analysis.

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/


This package contains the IEEE Computer Society subset of the full IEEEtran
package and is intended for use with IEEE Computer Society publications.
The included version of the IEEEtran_HOWTO.pdf has been specially formatted
in IEEE Computer Society (compsoc) journal mode.


For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for a IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf_compsoc.tex, bare_jrnl_compsoc.tex.
***************************************************************************


==> backup/01-relatedWork.tex <==
% \section{Related Work}

% The use of face images collected as part of border controls is restricted by the European General Data Protection Law to be processed for no other reason than its original
% purpose. This paper \cite{zhang2021applicability} investigates the suitability of synthetic face images generated with StyleGAN and StyleGAN2 to compensate for the urgent lack of publicly available large scale test data. This work analyses the differences between synthetically generated face images and real face images from the biometric perspective. The authors choose to assess the quality of the face images reflecting regular biometric systems where quality is first determined before using it for any biometric purpose. Face Quality Assessment Algorithms (FQAA) quantify the biometric quality of a sample (for instance, face image) by translating it to a quality score between [0, 100]. By measuring the face quality metrics of synthetically
% generated face samples, we can establish if they can be bused for biometric algorithm training and testing purposes. The main contribution of this paper is in investigating and reporting to which extent the synthetic samples could replace the need for real images for conducting biometric
% performance tests of a pre-trained face recognition system. More specifically, the goal is to obtain synthetic face images that are similar to real face images not only from the human perception point, but also in the context of face recognition. StyleGAN and StyleGAN2 are used to generate synthetic faces. Finally, we conclude that StyleGAN2 and FRGC images have shown the minor differences in face quality, which means the evaluated synthetic data can achieve a similar quality as biometric samples in EES cases and allows us to exploit both domains for realistic biometric performance tests. 
% \par The authors in \cite{aranjuelo2021key} argue that in some countries, there are privacy laws that limit the kind of data that can be recorded for specific tasks in an open scenario (e.g., face recognition). Some other tasks may involve
% capturing data in dangerous situations to develop intelligent systems, for example in the automotive industry. In addition, collecting a balanced dataset, which includes different situations or conditions (e.g., illumination), is an additional challenge that needs to be addressed. Even if all these difficulties are overcome, the need for labelled data involves an expensive and time-consuming annotation process, which can make the dataset gathering process unaffordable. For all these reasons, they generate different synthetic training datasets with particular features and use them to train a DNN for people detection in large spaces using omnidirectional cameras. Experimental results with real-world data show that proper synthetic data minimize the domain gap. We also show that expanding a training dataset to include synthetic samples in addition to real samples, can improve the model’s capabilities. 
% \par One of the challenges with regard to the social acceptance of eye tracking technology is however the preserving of sensitive and personal information. As it is possible to derive a lot of sensitive and personal information from eye tracking data such as intentions, behaviors,
% or fatigue since eyes are not fully controlled in a conscious way. To tackle this challenge, we employ a privacy preserving framework based on randomized encoding to train a Support Vector Regression model using synthetic eye images privately to estimate the human gaze. During the computation, none of the parties learn about the data or the result that any other party has. Furthermore, the party that trains the model cannot reconstruct pupil, blinks or visual scanpath. The experimental results show that our privacy-preserving framework is capable of working in realtime, with the same accuracy as compared to non-private version \cite{bozkir2020privacy}. According to a recent survey, people agree to share their eye tracking data only when it is co-owned by a governmental health-agency or is used for research purposes. This indicates that people are hesitant about sharing their eye tracking data in commercial applications. Therefore, there is a likelihood that larger communities could adopt HMDs or smart glasses if privacy-preserving techniques are applied in
% the eye tracking applications.

% \par Most of these approaches evaluate their performance on very small data sets or assume ideal distributions (that could differ significantly from the real data). Acquiring large biometric datasets for evaluation purposes is time consuming, expensive, and complicated with privacy issues. In this work \cite{osadchy2017g}, we present GENFACE, the first publicly available system for generating synthetic facial images. GENFACE can generate a large number of facial images that offers a solution to aforementioned problems. It can be used in many biometric applications such as face-based authentication systems, e.g., for the testing and evaluation phase. Another possible application of GENFACE is to offer the ability to balance the ROC curves with the error correction codes used in authentication systems employing secure sketch or fuzzy extractors. As a case study, we show how to use GENFACE in evaluating SecureFace, a face-based
% authentication system that offers end-to-end authentication and privacy. 
% \par Nowadays large-scale identity management systems enrol more than one billion data subjects. Effective testing of such biometric identification systems and biometric indexing approaches requires large datasets of biometric data. Currently, the size of the publicly available iris datasets is insufficient, especially for system scalability assessments. Synthetic data generation offers a potential solution to this issue. In \cite{drozdowski2017sic} we present a method for generation of synthetic binary iris-based templates, i.e. Iris-Codes, which are the de
% facto standard used throughout major biometric deployments around the world. We validate the statistical properties of the synthetic templates and show that they closely resemble ones produced from real ocular images.

% \par Touch dynamics is vulnerable to
% potential security attacks such as shoulder surfing, camera attack, and smudge attack. As a result, it is challenging to rule out genuine imposters while only relying on models that learn from real touchstrokes. In this paper \cite{deb2020use}, a touchstroke authentication model based on Auxiliary Classifier Generative Adversarial Network (AC-GAN) is presented. Given a small subset of a legitimate user's touchstrokes data during training, the presented AC-GAN model learns to generate a vast amount of synthetic touchstrokes that closely approximate the real touchstrokes, simulating imposter behavior, and then uses both generated and real touchstrokes in discriminating real user from the imposters. The presented network is trained on the Touchanalytics dataset and the discriminability is evaluated with popular performance metrics and loss functions. The evaluation results suggest that it is possible to achieve comparable authentication accuracies with Equal Error Rate ranging from 2\% to 11\% even when the generative model is challenged with a vast number of synthetic data that effectively simulates an imposter behavior. {\color{red}{Read again}}

% \par Pixel-wise crowd understanding is the most fundamental task in crowd analysis
% because of its finer results for video sequences or still images than other analysis tasks. Unfortunately, pixel-level understanding needs a large amount of labeled training data. An-
% notating them is an expensive work, which causes that current crowd datasets are small. As a result, most algorithms suffer from over-fitting to varying degrees. In \cite{wang2021pixel} Firstly, we develop a free data collector and labeler to generate synthetic and labeled crowd scenes in a computer game, Grand Theft Auto V. Then we use it to construct a large-scale, diverse synthetic crowd dataset. Secondly, we propose two simple methods to improve the performance of crowd understanding via exploiting the synthetic data. To be specific, (1) supervised crowd understanding: pre-train a crowd analysis model on the synthetic data, then fine-tune it using the real data and labels, which makes the model perform better on the real world; (2) crowd understanding via domain adaptation: translate the synthetic data to photo-realistic images, then train the model on translated data and labels. As a result, the trained model works well in real crowd scenes.

% \par Keystroke dynamics (KD) is a behavioral biometric modality that allows the authentication of individuals through their way of typing a password or a free text on a keyboard \cite{migdal2019statistical}. However, collecting such sensitive data is also very time consuming and constrained, s.a. GDPR legislation in Europe. In the case of keystroke dynamics, most existing databases have less than 200 users. For these reasons, it is crucial for this biometric modality to be able to generate a significant and realistic synthetic dataset of keystroke dynamics samples. We propose in this paper an original approach for the generation of synthetic keystroke data given samples from known users as a first step towards the generation of synthetic datasets. Experimental results show the capability of the proposed statistical model to generate realistic samples from existing datasets in the literature. 

% \par In speech recognition problems, data scarcity often poses an issue due to the willingness of humans to provide large amounts of data for learning and classification. In this work, we take a set of 5 spoken Harvard sentences from 7 subjects and consider their MFCC attributes. Using character level LSTMs (supervised learning) and OpenAI’s attention-based GPT-2 models, synthetic MFCCs are generated by learning from the data provided on a per-subject basis. A neural network is trained to classify the data against a large dataset of Flickr8k speakers and is then compared to a transfer learning network performing the same task but with an initial weight distribution
% dictated by learning from the synthetic data generated by the two models. The best result for all of the 7 subjects were networks that had been exposed to synthetic data, the model pre-trained
% with LSTM-produced data achieved the best result 3 times and the GPT-2 equivalent 5 times (since one subject had their best result from both models at a draw). Through these results, we argue that speaker classification can be improved by utilising a small amount of user data but with exposure to synthetically generated MFCCs which then allow the networks to achieve near
% maximum classification scores \cite{bird2020lstm}.


% \par The restrictions posed by the recent trans-border regulations to the usage of biometric data force researchers in the fields of digitized forensics and biometrics to use synthetic data for development and evaluation of new algorithms. For digitized forensics, we introduce a technique for conversion of privacy-sensitive datasets of real latent fingerprints to "privacy-friendly" datasets of synthesized fingerprints. Privacy-friendly means in our context that the generated fingerprint images cannot be linked to a particular person who provided fingerprints to the original dataset. In contrast to the standard fingerprint generation approach that makes use
% of mathematical modeling for drawing ridge-line patterns, we propose applying a data-driven approach making use of generative adversarial neural networks (GAN). In our synthesis experiments \cite{seidlitz2021generation} the performance of three established GAN architectures is examined. The NIST Special Database 27 is exemplary used as a data source of real latent fingerprints. The set of training images is augmented by applying filters from the
% StirTrace benchmarking tool. The suitability of the generated fingerprint images is checked with the NIST fingerprint image quality tool (NFIQ2). The unlinkability to any original fingerprint is established by evaluating outcomes of the NIST fingerprint matching tool. 
% \par The research in biometric recognition using hand shape has been somewhat stagnating in the last decade. Meanwhile, computer vision and machine learning have experienced a paradigm shift with the renaissance of deep learning, which has set the new state-of-the-art in many related fields. Inspired by successful applications of deep learning for other biometric modalities, we \cite{svoboda2020clustered} propose a novel approach to 3D hand shape recognition from RGB-D data based on geometric deep learning techniques. We show how to train our model on synthetic data and retain the performance on real samples during test time. To evaluate our method, we provide a new dataset NNHand RGBD of short video sequences and show encouraging performance compared to diverse baselines on the new data, as well as current benchmark dataset HKPolyU. Moreover, the new dataset opens door to many new research directions in hand shape recognition. 

% \par In \cite{yadav2019synthesizing}, the authors utilize the generative capability of a Relativistic Average Standard Generative Adversarial Network (RaSGAN) to synthesize high quality images of the iris. Furthermore, we demonstrate the viability of using these synthetic images to train a PAD system that can generalize well to unseen attacks.

% \par Soft-Biometric information, such as gender, has great potential for applications in security, forensics and marketing. Unfortunately, there are few gender-labelled databases available which make state of the art techniques, such as deep learning, difficult to use. An alternative source of data to train these algorithms are synthetic images. In \cite{tapia2019soft}, a novel GAN-based algorithm that preserves gender information while generating synthetic images is presented. It uses a latent vector that encodes gender information within the conditional GAN algorithm. Resulting synthetic images were tested
% using a gender classifier algorithm (CNN). Experiments demonstrate that the proposed method can be a useful tool for the synthesis of gender-labelled images to be used in training Deep Learning gender-classification algorithms. Furthermore, when using this dataset alongside the GFI-UND dataset (or the UNAB-Gender dataset), gender-classification rates were improved by 10\% with respect to the original database. These improved rates demonstrate that synthetic NIR periocular iris images will be a useful tool for training Deep Learning algorithms for gender classification.

% \par Electrocardiograph (ECG) has been well proved to contain adequately unique patterns for individual recognition and considered as a promising biometric which is hard to spoof
% and forge because of its intrinsic liveness detection and dynamic variance. In
% \cite{gao2018replicating}, we present a new presentation attack method that can spoof the target authentication system by generating a sufficiently large number of high-quality fake ECG samples based upon the public datasets and limited attempt efforts. Our approach
% combines the cluster-based template searching, off-line substitute classifier training, data synthesis, and VAE-based counterfeits generation. Considering a robust ECG authentication system with effective replay detection mechanism that can effectively identify and reject common noise injection attacks, experimental results show that the fake ECG samples generated by our approach can achieve an average acceptance rate of 95%,
% compared with the best acceptance rate of 39\% for noise-injected fake samples. We explored the vulnerability of the ECG biometric authentication system and proposed a black-box presentation attack relying on the limited access efforts and feedback labels from the unknown verification classifier. Leveraging the public databases, we first obtained 8 accepted substitute ECG samples and selected 100 samples from the database based on the similarity ranking. Then we synthesized more fake samples using CFM and autoencoder to train a generative model, VAE. For each of the 5 users with different EER levels, 5,000 counterfeit ECG samples were generated from VAE (theoretically, infinite new samples can be generated). The results show that the fake samples can successfully pass through the verification of the target authentication system and the enhanced replay detectors, with very high acceptance rates cross all 5 genuine users. In summary, our approach possesses a much higher success rate than the noise injection attacks and demands much less attempt efforts than the brute-force attacks, under the same condition. 

% \par It is well known that deep learning approaches to face recognition suffer from various biases in the available training data. In \cite{kortylewski2019analyzing}, we demonstrate the large potential of synthetic data for analyzing and reducing the negative effects of dataset bias on deep face recognition systems. In particular we explore two complementary application areas for synthetic face images: 1) Using fully annotated synthetic face images we can study the face recognition rate as a function of interpretable parameters such as face pose. This enables us to systematically analyze the effect of different types of dataset biases on the generalization ability of neural network architectures. Our analysis reveals that deeper neural network architectures can generalize better to unseen face poses. Furthermore, our study shows that current neural network architectures cannot disentangle face pose and facial identity, which limits their generalization ability. 2) We pre-train neural networks with large-scale synthetic data that is highly variable in face pose and the number of facial identities. After a subsequent fine-tuning with real-world data, we observe that the damage of dataset bias in the real-world data is largely reduced.  

% \par Currently, the large number of interesting researches based on the analysis of the VoxCeleb1 and VoxCeleb2 datasets are published. High results are obtained using huge architectures:
% ResNet18, ResNet34, ResNet50. They are not suitable for our purpose because we are considering only a small part of the VoxCeleb1 dataset, which is less than 5\% of the total volume. If you apply deep architectures to the small dataset, the network will be overfitting and have weak generalization ability \cite{anton2020modification}. The voice recognition results show that the percent of correct answers on the training dataset is 99.84\%, but the score on the verification set is 60.89\%, and on the test set is 51.55\%. The result indicates that the model is overfitting and it has a low generalizing ability. In this research, audio data was changed with using different transformations that we earlier described in the current article. Using the method of synthetic augmentation allowed us to improve the score. 

% \par A new method to generate synthetic swipe gestures using Generative Adversarial
% Networks and samples acquired during real human-device interaction. This method
% allows to generate synthetic samples that mimic the human behaviour \cite{acien2020becaptcha}. A new bot detection approach based on modelling the user behaviour in smartphone interaction using multiple inbuilt sensors: BeCAPTCHA. We improve the bot detection accuracy training with real and synthetic samples generated with the adversarial method proposed.

% \par In \cite{friedman2017synthetic}, the authors create synthetic biometric databases to
% study general, fundamental, biometric principles. First, we check the validity of the synthetic database design by comparing it to real data in terms of biometric performance. The real data
% used for this validity check was from an eyemovement related biometric database. Next, we
% employ our database to evaluate the impact of
% variations of temporal persistence of features on
% biometric performance. We index temporal
% persistence with the intraclass correlation
% coefficient (ICC). We find that variations in
% temporal persistence are extremely highly
% correlated with variations in biometric
% performance. Finally, we use our synthetic
% database strategy to determine how many
% features are required to achieve particular levels of performance as the number of subjects in the database increases from 100 to 10,000. An
% important finding is that the number of features
% required to achieve various EER values (2\%,
% 0.3\%, 0.15\%) is essentially constant in the
% database sizes that we studied. We hypothesize
% that the insights obtained from our study would
% be applicable to many biometric modalities
% where extracted feature properties resemble the
% properties of the synthetic features we discuss in this work. 

% \par In \cite{han2018improving}, the authors provide a synthetic data generator methodology with fully controlled, multifaceted variations
% based on a new 3D face dataset (3DU-Face). We customized synthetic datasets to address specific types of variations (scale, pose, occlusion, blur, etc.), and systematically investigate the influence of different variations on face detection performances. We examine whether and how these factors contribute to better face detection performances.  

% \par  Creating and labeling data can be extremely time consuming and labor intensive. For this reason, lack of sufficiently large datasets for training deep structures is often noted
% as a major obstacle and instead, synthetic data generation is proposed. With their high acquisition and labeling complexity, this also applies to fingerprints. In the literature, a number of synthetic fingerprint generation systems have been proposed, but mostly for algorithm evaluation purposes. In this paper \cite{irtem2019impact}, we aim to analyze the use of synthetic fingerprint data with different levels of degradation for training deep neural networks. Fingerprint classification problem is selected as a case-study and the experiments are conducted on a public domain database, NIST SD4. A positive correlation between the synthetic data
% variation and the classification rate is observed while achieving state-of-the-art results.

% \par The most accurate head pose estimators
% are based on Deep Neural Networks that are trained with the supervised approach and rely primarily on the accuracy of training data. The acquisition of real head pose data with a wide variation of yaw, pitch and roll is a challenging task. Publicly available head pose datasets have limitations with respect to size, resolution, annotation accuracy and diversity. In this work \cite{basak2021learning}, a methodology is proposed to generate pixel-perfect synthetic 2D headshot images rendered from high-quality 3D synthetic facial models with accurate head pose annotations. A diverse range of variations in age, race, and gender are also provided. The resulting dataset includes more than 300k pairs of RGB images with corresponding head pose annotations. A wide range of variations in pose, illumination and background are included. The dataset is evaluated by training a state-of-the-art head pose estimation model and testing against the popular evaluation-dataset Biwi. The results show that training with purely synthetic data generated using the proposed methodology achieves close to state-of-the-art results on head pose estimation which are originally trained on real human facial datasets. As there is a domain gap between the synthetic images and real-world images in the feature space, initial experimental results fall short of the current state-of-the-art. To reduce the domain gap, a semisupervised visual domain adaptation approach is proposed, which simultaneously trains with the labelled
% synthetic data and the unlabeled real data. When domain adaptation is applied, a significant improvement in model performance is achieved. Additionally, by applying a data fusion-based transfer learning approach, better results are achieved than previously published work on this topic. 

% \par Autonomous speaker identification suffers issues of data scarcity due to it being unrealistic to gather hours of speaker
% audio to form a dataset, which inevitably leads to class imbalance in comparison to the large data availability from non-speakers since large-scale speech datasets are available online. In this study \cite{bird2020overcoming}, we explore the possibility of improving speaker recognition by augmenting the dataset with synthetic data produced by training a Character-level Recurrent Neural Network on a short clip of five spoken sentences. A deep neural network is trained on a selection of the Flickr8k dataset as well as the real and synthetic speaker data (all in the form of MFCCs) as a binary classification problem in order to discern the speaker from the Flickr speakers. Ranging from 2,500 to 10,000 synthetic
% data objects, the network weights are then transferred to the original dataset of only Flickr8k and the real speaker data, in order to discern whether useful rules can be learnt from the synthetic data. Results for all three subjects show that fine-tune learning from datasets augmented with synthetic speech improve
% the classification accuracy, F1 score, precision, and the recall when applied to the scarce real data vs non-speaker data. We conclude that even with just five spoken short sentences, data
% augmentation via synthetic speech data generated by a CharRNN can improve the speaker classification process. Accuracy and related metrics are shown to improve from around 93\% to
% 99\% for three subjects classified from thousands of others when fine-tuning from exposure to 2500-1000 synthetic data points. High F1 scores, precision and recall also show that issues due to
% class imbalance are also solved. 

% \par This brief survey \cite{yanushkevich2006synthetic} addresses the state-of-the-art techniques of inverse biometrics, which deals with synthesis of biometric data. It reports on genesis of synthetic biometric, advanced methods, and open application-specific problems. Currently deployed biometric systems use comprehensive methods and algorithms (such as pattern recognition, decision making, database searching, etc.) to analyze biometric data collected from individuals. We consider the inverse task, synthesis of artificial biometric data. These biologically meaningful data are useful, for example, for testing the biometric tools, and for enhancing the security of biometric systems. The synthetic data replicate all possible instances of otherwise unavailable data, thus, creating a variety of samples for testing. Properly created artificial biometric data provides a basis for enhancing security through the detailed and controlled modeling of a wide range of training skills, strategies and tactics of a hypothetical robber or forger. Databases of synthetic biometric data also serve for simulation in forensic systems. 

% \par  In the case of keystroke dynamics,
% existing databases have less than 200 users. For these reasons, we aim at generating a keystroke dynamics synthetic dataset. This paper presents the generation of keystroke data from known users as a first step towards the generation of synthetic datasets, and could also be used to impersonate users’ identity \cite{migdal2018analysis}. We think this work is important, because it is known that KD studies are not fair as (i) acquisition protocols are different between studies; (ii) there
% is not always a comparative study when authors
% propose new algorithms; and (iii) there are not always a valuable statistical evaluation. Our work contributes to solve these problems. 

% \par we propose to automatically create a large-scale synthetic gait dataset (called VersatileGait) by a game engine, which consists of around one million silhouette sequences of 11,000 subjects with fine-grained attributes in
% various complicated scenarios \cite{dou2021versatilegait}. Compared with existing real gait datasets with limited samples and simple scenarios, the proposed VersatileGait dataset possesses several nice properties, including huge dataset size, high sample diversity, high-quality annotations, multi-pitch angles, small domain gap with the real one, etc. Furthermore, we investigate the effectiveness of our dataset (e.g., domain transfer after pretraining). Then, we use the fine-grained attributes from VersatileGait to promote gait recognition in both accuracy and speed, and meanwhile justify the gait recognition
% performance under multi-pitch angle settings. Additionally, we explore a variety of potential applications for research. Extensive experiments demonstrate the value and effectiveness of the proposed VersatileGait in gait recognition along
% with its associated applications. We will release both VersatileGait and its corresponding data generation toolkit for further studies.
 
%  \par  In this paper \cite{hu2017deceive}, we propose a mouse movement simulation method to inspect the vulnerability of this authentication technique. The authenticity of the mouse movement data generated by the simulation method is validated by five benchmark classifiers. Experimental results show the simulation method possesses a high authentication pass rate for most users. It indicates the proposed method can simulate real user mouse actions and the persuasive assumption that mouse behavior is difficult to imitate might be too optimistic.
 
%  \par In this paper \cite{piplani2018faking}, we empirically demonstrate the vulnerability of a passthought authentication system to fake signals generated by Generative Adversarial Networks (GANs), and use these same signals to make authenticators more robust. We first train a classifier that is able to authenticate a subject based on their EEG signals. The classifier performs a binary classification task: either the user is who they claim to be, or not. To test the robustness of the authenticator against attacks we train a GAN to generate signals that mimic the EEG signals of the “positive” subject. We find that a well-trained GAN is able to generate signals that the classifier consistently accepts. To alleviate this vulnerability, we re-train the classifier with this GAN generated data. We find that the classifier re-trained against synthetic data is both more robust against this attack, and more accurate in accepting real data than the initial classifier.

% \par In this research \cite{yadav2020relativistic}, we propose a presentation attack detection (PAD) method that utilizes a discriminator that is trained to distinguish between bonafide iris images and synthetically generated iris images. We hypothesize that such a discriminator will generate a tight boundary around the bonafide samples. This would allow the discriminator to
% better separate the bonafide samples from all types of PA samples. For generating synthetic irides, we train the Relativistic Average Standard Generative Adversarial Network (RaSGAN) that has been shown to generate higher resolution and better quality images than standard GANs. The relativistic discriminator (RD) component of the trained RaSGAN is then appropriated for PA detection and is referred
% to as RD-PAD. 

% \par In this paper \cite{buriro2021swipegan},
% we propose SwipeGAN - to generate swiping samples to be used for smartphone user authentication. Extensive experimentation and evaluation show the quality of the generated synthetic swiping samples and their efficacy in increasing the accuracy of the authentication scheme.

% \par New methods for generating synthetic handwriting images for biometric applications have recently been developed. The temporal evolution of handwriting from childhood to adulthood is usually left unexplored in these works. This paper \cite{carmona2017temporal} proposes a novel methodology for including temporal evolution in a handwriting synthesizer by means of simplifying the text trajectory plan and handwriting dynamics. This is achieved through a tailored version of the kinematic theory of rapid human movements and the neuromotor inspired handwriting synthesizer. The realism of the proposed method has been evaluated by comparing the temporal evolution of real and synthetic samples both quantitatively and subjectively. The quantitative test is based on a visual perception algorithm that compares the letter variability and the number of strokes in the real and synthetic handwriting produced at different ages. In the subjective
% test, 30 people are asked to evaluate the perceived realism of the evolution of the synthetic handwriting. 

% \par This work \cite{morales2015synthesis} proposes and analyzes a novel methodology for hand-shape image synthesis. The hand-shape is
% a popular biometric trait with a high convenience of use and non-intrusive acquisition. The proposed algorithm allows to generate realistic images with natural intra-person and inter-person variability. The method is based on the Active Shape Model algorithm which has been modified in order to add the biometric information typical of new synthetic identities. The generated images are evaluated using three public databases and two hand-shape recognition systems. The results show the suitability of the synthetic data for biometric recognition works. In addition, two novel applications have been proposed to provide new insights in hand-shape biometric recognition including: improvement of machine learning classification based on synthetic training sets and scalability analysis of hand-shape biometrics when the population of the database is increased by two orders of magnitude with respect to existing databases.

% \par This paper \cite{gouiaa2017learning} presents a system for human posture recognition using a camera and two infrared light sources. It uses as input the combination of the body silhouette and its (invisible to the eye) cast shadows. Conventional video-surveillance methods based on a single camera can fail to infer the correct posture since different postures can look similar under perspective projection. Fortunately, cast body shadows, generated by infrared lights, offer additional posture information that cannot be directly captured by a single camera. Each shadow can be projected on different surfaces (e.g. floor, walls, and furniture) generating complex body projections that represent various shapes within the same posture class. These shadow images are very challenging and difficult to describe with traditional handcrafted features that need to be somewhat invariant to these within-class changes. However, a deep convolution neural network (CNN) is able to learn a better data representation from a large-scale dataset. In the absence of a big real dataset, we propose to use synthetic data for training the CNN classifier. Learning from synthetic data is a challenging task due to the gap between synthetic and real feature distributions. Thus, we propose a normalization technique to bridge the gap and help the classifier to better generalize with real data. We evaluated the proposed system on a new real dataset captured in our laboratory and a simulated dataset generated with computer graphics tools. Experimental results validated the efficiency of the CNN model against other conventional methods. Furthermore, the combination of cast shadows and body silhouette had better performance than using only the body silhouette as expected. 

% \par Augmented and virtual reality deployment is finding increasing use in novel applications. Some of these emerging and foreseen applications allow the users to access sensitive information and functionalities. Head Mounted Displays (HMD) are used to enable such applications and they typically include eye facing cameras to facilitate advanced user interaction. Such integrated cameras capture iris and partial periocular region during the interaction. This work \cite{boutros2020iris} investigates the possibility of using the captured ocular images from integrated cameras from HMD devices for biometric verification, taking into account the expected limited computational power of such devices. Such an approach can allow user to be verified in a manner that does not require any special and explicit user action. In addition to our comprehensive analyses, we present a light weight, yet accurate, segmentation solution for the ocular region captured from HMD devices. Further, we benchmark a number of well-established iris and periocular verification methods along with an in-depth analysis on the impact of iris sample selection and its effect on iris recognition performance for HMD devices. To the end, we also propose and validate an identity preserving synthetic ocular image generation mechanism that can be used for large scale data generation for training purposes or attack generation purposes. We establish the realistic image quality of generated images with high fidelity and identity preserving capabilities through benchmarking them for iris and periocular verification.

% \par In this work \cite{ruiz2020off}, we propose the use of Siamese Neural Networks to help solve the off-line handwritten signature verification problem with random forgeries in a writer-independent context. Our proposed solution can be used on new signers without the need for any additional training. Also, we have analyzed
% three types of synthetic data to increase the amount of samples and the variability needed for training deep neural networks: augmented data samples from GAVAB dataset, a proposal of compositional synthetic signature generation from shape primitives and the GPDSSynthetic dataset. The first two approaches are “on-demand” generators and they can be used during the training stage to produce a potentially infinite number of synthetic signatures. In our approach, we initially trained Siamese Neural Networks using signatures from GAVAB dataset and different combinations of synthetic data. The best
% verification results were obtained when combining original and synthetic signatures for training. Additionally, we tested our approach on the GPSSynthetic, MCYT, SigComp11 and CEDAR datasets demonstrating the generalization capabilities of our proposal.

% \par Fast and robust three-dimensional reconstruction of facial geometric structure from a single image is a challenging task with numerous applications. Here \cite{richardson20163d}, we introduce a learning-based approach for reconstructing a threedimensional face from a single image. Recent face recovery methods rely on accurate localization of key characteristic points. In contrast, the proposed approach is based on a Convolutional Neural Network (CNN) which extracts the face geometry directly from its image. Although such deep architectures outperform other models in complex computer vision problems, training them properly requires a large dataset of annotated examples. In the case of three dimensional faces, currently, there are no large volume datasets, while acquiring such big-data is a tedious task. As an alternative, we propose to generate random, yet nearly photo-realistic, facial images for which the geometric form is known. The suggested model successfully recovers facial shapes from real images, even for faces with extreme expressions and under various lighting conditions.

% \par There are several confounding factors that can reduce the accuracy of gait recognition systems. These factors can reduce the distinctiveness, or alter the features used to characterise gait; they include variations in clothing, lighting, pose and environment, such as the walking surface. Full invariance to all confounding factors is challenging in the absence of high-quality labelled training data. We introduce a simulation-based methodology \cite{charalambous2016data} and a subject-specific dataset which can be used for generating synthetic video frames and sequences for data augmentation. With this methodology, we generated a multi-modal dataset. In addition, we supply simulation files that provide the ability to simultaneously sample from several confounding variables. The basis of the data is real motion capture data of subjects walking and running on a treadmill at different speeds. Results from gait recognition experiments suggest that information about the identity of subjects is retained within synthetically generated examples. The dataset and methodology allow studies into fully-invariant identity recognition spanning a far greater number of observation conditions than would otherwise be possible. 

% \par Reliability and accuracy of iris biometric modality has prompted its large-scale deployment for critical applications such as border control and national ID projects. The extensive growth of iris recognition systems has raised apprehensions about susceptibility of these systems to various attacks. In the past, researchers have examined the impact of various iris presentation attacks such as textured contact lenses and print attacks. In this research \cite{kohli2017synthetic}, we present a novel presentation attack using deep learning based synthetic iris generation. Utilizing the generative capability of deep convolutional generative adversarial networks and iris quality metrics, we propose a new framework, named as iDCGAN (iris deep convolutional generative adversarial network) for generating realistic appearing synthetic iris images. We demonstrate the effect of these synthetically generated iris images as presentation attack on iris recognition by using a commercial system. The state-of-the-art presentation attack detection framework, DESIST is utilized to analyze if it can discriminate these synthetically generated iris images from real images. The experimental results illustrate that mitigating the proposed synthetic presentation attack is of paramount importance.
 

% \par Recent advances in deep learning have significantly increased the performance of face recognition systems. The performance and reliability of these models depend heavily on the
% amount and quality of the training data. However, the collection of annotated large datasets does not scale well and the control over the quality of the data decreases with the size of the dataset. In this work \cite{kortylewski2018training}, we explore how synthetically generated data can be used to decrease the number of real-world images needed for training deep face recognition systems. In particular, we make use of a 3D morphable face model for the generation of images with arbitrary amounts of facial identities and with full control over image variations, such as pose, illumination, and background. In our experiments with an off-the-shelf face recognition software we observe the following phenomena: 1) The amount of real training data needed to train competitive deep face recognition systems can be reduced significantly. 2) Combining large-scale real-world data with synthetic data leads to an increased performance. 3) Models trained only on synthetic data with strong variations in pose, illumination, and background perform very well across different datasets even without dataset adaptation. 4) The realto-virtual performance gap can be closed when using synthetic data for pre-training, followed by fine-tuning with real-world images. 5) There are no observable negative effects of pretraining with synthetic data. Thus, any face recognition system in our experiments benefits from using synthetic face images. The synthetic data generator, as well as all experiments, are publicly
% available. 

% \par In this paper \cite{trigueros2018generating} we investigate the feasibility of using synthetic data to augment face datasets. In particular, we propose a novel generative adversarial network (GAN) that can disentangle identity-related attributes from non-identity-related attributes. This is done by training an embedding network that maps discrete identity labels to an identity latent space that follows a simple prior distribution, and training a GAN conditioned on samples from that distribution. Our proposed GAN allows us to augment face datasets by generating both synthetic images of subjects in the training set and synthetic images of new subjects not in the training set. By using recent advances in GAN training, we show that the synthetic images generated by our model are photo-realistic, and that training with augmented datasets can indeed increase the accuracy of face recognition models as compared with models trained with real images alone. 

% \par Using data generated by generative adversarial networks or three-dimensional (3D) technology for face recognition training is a theoretically reasonable solution to the problems of unbalanced data distributions and data scarcity. However, due to the modal difference between synthetic data and real data, the direct use of data for training often leads to a decrease in the recognition performance, and the effect of synthetic data on recognition remains ambiguous. In this paper \cite{zhai2021demodalizing}, after observing in experiments that modality information has a fixed form, we propose a demodalizing face recognition training architecture for the first time and provide a feasible method for recognition training using synthetic samples. Specifically, three different demodalizing training methods, from implicit to explicit, are proposed. These methods gradually reveal a generated modality that is difficult to quantify or describe. By removing the modalities of the synthetic data, the performance degradation is greatly alleviated. We validate the effectiveness of our approach on various benchmarks of large scale face recognition and outperform the previous methods, especially in the low FAR range.

% \par Over the past few years, Generative Adversarial Networks (GANs) have been receiving attention from image and time series domain. In this work \cite{chen2019emotionalgan}, we propose a novel sequence based generative model to  generate  ECG  samples  for  enhancing  emotion  state classification. Firstly, emotional related features are extracted to represent emotion state in ECG record. Secondly, random forest and support vector machine are trained to  classify arousal and valence  states. Then  proposed  generative  model  is  applied  to generate ECG sample with the corresponding emotion state label. Finally, synthetic data is used to augment the original training set for another classification. Our proposed model classifying emotion state  in  both  arousal  and  valence  domain.  With  synthetic augmented dataset, the average classification accuracy increases around 5\%  compared  with  using  only  original  data.  The  result demonstrates the notable effectiveness of our generative model for enhancing emotion state classification. 


% \par cognitive impairment is one of the crucial problems elderly   people   face.   Tracking   their   daily   life activities   and detecting early indicators of cognitive decline would be necessary for   further   diagnosis.   Depending   on   the   decline   magnitude, monitoring  may  need  to  be  done  over  long  periods  of  time to  detect  abnormal  behaviour.  In  the  absence  of  training  data,it  would  be  helpful  to  learn  the  normal  behaviour  and  daily life  patterns  of  a  (cognitively)  healthy  person  and  use  them  as a  basis  for  tracking  other  patients.  In  this  paper \cite{arifoglu2019abnormal},  we  propose to  investigate  Recursive  Auto-Encoders  (RAE)-based  transfer learning  to  cope  with  the  problem  of  scarcity  of  data  in  the context  of  abnormal  behaviour  detection.  We  present  a  method for generating synthetic data to reflect on some behavior of people with  dementia.  An  RAE  model  is  trained  on  data  of  a  healthy person  in  a  source  household.  Then,  the  resulting  RAE  is  used to  detect  abnormal  behavior  in  a  target  house.  To  evaluate  the proposed  approach,  we  compare  the  results  with  the-state-of-the-art  supervised  methods.  The  results  indicate  that  transfer learning is promising when there is lack of training data. 

% \par As Consumer Technologies (CT) seeks to engage and interact more closely with the end-user it becomes important to observe and  analyze a user’s  interaction  with CT  devices  and associated services. One of the most useful modes for monitoring a user is to analyze a real-time video stream of their face. Facial expressions,  movements  and  biometrics  all  provide  important information, but obtaining a calibrated input with 3D accuracy from a single camera requires accurate knowledge of the facial depth and distance of different features from the camera. In this paper \cite{khan2021accurate}, a method is proposed to generate synthetic high-accuracy  human  facial  depth  from  synthetic  3D  face models. The generated synthetic human facial dataset is then used in Convolutional Neural Networks (CNN’s) for monocular depth facial estimation and the results of the experiments are presented.

% \par Monitoring of protected areas to curb illegal activitieslike poaching and animal trafficking is a monumental task.T o augment existing manual patrolling efforts, unmannedaerial surveillance using visible and thermal infrared (TIR)cameras is increasingly being adopted. Automated data ac-quisition has become easier with advances in unmannedaerial vehicles (UAVs) and sensors like TIR cameras, whichallow surveillance at night when poaching typically occurs.However, it is still a challenge to accurately and quicklyprocess large amounts of the resulting TIR data. In this pa-per \cite{bondi2020birdsai}, we present the first large dataset collected using a TIRcamera mounted on a fixed-wing UAV in multiple Africanprotected areas. This dataset includes TIR videos of hu-mans and animals with several challenging scenarios likescale variations, background clutter due to thermal reflec-tions, large camera rotations, and motion blur. Addition-ally, we provide another dataset with videos synthetically generated with the publicly available Microsoft AirSim sim-ulation platform using a 3D model of an African savannaand a TIR camera model. Through our benchmarking ex-periments on state-of-the-art detectors, we demonstrate thatleveraging the synthetic data in a domain adaptive settingcan significantly improve detection performance. We alsoevaluate various recent approaches for single and multi-object tracking.  With the increasing popularity of aerialimagery for monitoring and surveillance purposes, we an-ticipate this unique dataset to be used to develop and eval-uate techniques for object detection, tracking, and domainadaptation for aerial, TIR videos.


% \par A    large    amount    of    training   data   is    usuallycrucial  for  successful  supervised  learning.  However,  the  task  ofproviding  training  samples  is  often  time-consuming,  involvinga  considerable  amount  of  tedious  manual  work.  In  addition,the  amount  of  training  data  available  is  often  limited.  As  analternative,  in  this  paper \cite{feng2015cascaded},  we  discuss  how  best  to  augment  theavailable  data  for  the  application  of  automatic  facial  landmarkdetection.  We  propose  the  use  of  a  3D  morphable  face  modelto  generate  synthesized  faces  for  a  regression-based  detectortraining.  Benefiting  from  the  large  synthetic  training  data,  thelearned detector is shown to exhibit a better capability to detectthe  landmarks  of  a  face  with  pose  variations.  Furthermore,  thesynthesized  training  data  set  provides  accurate  and  consistentlandmarks  automatically  as  compared  to  the  landmarks  anno-tated manually, especially for occluded facial parts. The syntheticdata and real data are from different domains; hence the detectortrained  using  only  synthesized  faces  does  not  generalize  well  toreal  faces.  To  deal  with  this  problem,  we  propose  a  cascadedcollaborative  regression  algorithm,  which  generates  a  cascadedshape  updater  that  has  the  ability  to  overcome  the  difficultiescaused  by  pose  variations,  as  well  as  achieving  better  accuracywhen  applied  to  real  faces.  The  training  is  based  on  a  mix  of synthetic  and  real  image  data  with  the  mixing  controlled  bya  dynamic  mixture  weighting  schedule.  Initially,  the  traininguses  heavily  the  synthetic  data,  as  this  can  model  the  grossvariations  between  the  various  poses.  As  the  training  proceeds,progressively  more  of  the  natural  images  are  incorporated,  asthese can model finer detail. To improve the performance of theproposed  algorithm  further,  we  designed  a  dynamic  multi-scalelocal feature extraction method, which captures more informativelocal  features  for  detector  training.  An  extensive  evaluation  onboth controlled and uncontrolled face data sets demonstrates themerit  of  the  proposed algorithm.


% \par The finger-vein biometric offers a higher  degree of security, personal privacyand strong anti-spoofing capabilities than most other biometric modalities employed today. Emerging privacy concerns with the database acquisition and lack of availability of large scale finger-vein databases have posed challenges in exploring this technology for large scale applications. This paper \cite{hillerstrom2014generation} details the first attempt to synthesize finger-vein images and presents analysis of synthesized images for the biometrics authentication. We generate a database of 50,00 0 finger-vein images, corresp onding to 5000 different subjects,  with 10 different synthesized finger-vein images from each of the subject.  We use tractable probability models to compare synthesized finger-vein images with the real finger-vein images for their image variability .This paper also presents matching accuracy using the synthesized finger-vein database from 5000 different subjects, using 225,000 genuine and 1249,750,000 impostor matching scores, which suggests significant promises from finger-vein biometric modality for the large scale biometrics applications.



% \par This   work proposes   a sclera vessel texture   pattern   synthesis technique. As  it  is  difficult  to produce a a  large-scale collection of real  sclera data,synthetic  data can be a useful alternative  for researchers. Scleratexture was  synthesized  by a  non-parametric  basedtexture  regeneration  technique \cite{das2017sclera}.  A small  number  of  classes  from the UBIRIS  version:  1dataset  was  employed  as primitive  images.  Anappreciable result  wasachieved which demonstratesthesuccessful synthesisof sclera texture patterns.


% \par Monocular 3D facial shape reconstruction from a single2D facial image has been an active research area due to its wide applications.  Inspired by the success of deep neural networks (DNN), we propose a DNN-based approach for End-to-End 3D FAce Reconstruction (UH-E2FAR) from a single 2D image.  Different from recent works that reconstruct and refine the 3D face in an iterative manner usingboth an RGB image and an initial 3D facial shape rendering,  our DNN model \cite{dou2017end} is end-to-end, and thus the complicated 3D rendering process can be avoided.  Moreover, we integrate in the DNN architecture two components, namely a multi-task loss function and a fusion convolutional neural network (CNN) to improve facial expression reconstruction.With the multi-task loss function, 3D face reconstruction is divided into neutral 3D facial shape reconstruction and expressive 3D facial shape reconstruction. The neutral 3D facial shape is class-specific.  Therefore, higher layer features are useful.  In comparison, the expressive 3D facial shape favors lower or intermediate layer features. With the fusion-CNN, features from different intermediate layers are fused and transformed for predicting the 3D expressive facial shape. Through extensive experiments, we demonstrate the superiority of our end-to-end framework in improving the accuracy of 3D face reconstruction.

% \par Robust fingerprint pre-alignment is vital for identifi-cation systems and biometric cryptosystems based on fingerprintminutiae, where computation of a relative alignment by compa-rison of the fingerprints is inefficient or intractable, respectively.The  pre-alignment  is  achieved  through  an  absolute  alignment,i. e.  an  alignment  computed  for  each  fingerprint  independently,which can be applied for fingerprint registration to compensate for variations in the placement (translation) and rotation of thefingerprints prior to their comparison. In  this  work \cite{dieckmann2019fingerprint},  a  deep  learning  approach  for  absolute  pre-alignment  of  fingerprints  is  presented.  The  proposed  algorithmemploys a siamese network (with CNNs as subnetworks) whichis trained on synthetically generated fingerprints using horizon-tal/vertical  translation  and  rotation  as  three  regression  coefficients. Evaluations are conducted on the FVC2000 DB2a and theMCYT  fingerprint  database.  Compared  to  other  published  fingerprint pre-alignment methods, the presented scheme achieves higher accuracy w. r. t. rotation estimation and overall robustness.In  addition,  the  proposed  pre-alignment  is  applied  as  a  pre-processing step in a Fuzzy Vault scheme.

% \par Methods for generating synthetic data have become of  increasing  importance  to  build  large  datasets  required  for Convolution   Neural   Networks   (CNN)   based   deep   learning techniques for a wide  range  of  computer  vision  applications. In this  work,  we  extend existing methodologies  to  show  how  2D thermal  facial  data  can  be  mapped  to  provide  3D  facial  models.For  the proposed  research  work \cite{farooq2020generating} we  have  used  tufts  datasets  for generating 3D varying face  poses by  using a single frontal  face pose. The system works by refining the existing image quality by performing fusion  based image preprocessing  operations.  The refined outputs have better contrast adjustments, decreased noise level  and  higher exposedness  of  the  dark  regions.    It  makes  the facial  landmarks  and temperature  patterns  on  the  human  face more discernible and visible when compared to original raw data. Different  image  quality  metrics  are  used  to  compare  the  refined version of images with original images. In the next phase of the proposed study,the refined version of images is used to create 3D facial geometry structures by using Convolution Neural Networks (CNN).  The  generated  outputs  are  then  imported  in blender software  to  finally  extract  the  3D thermal  facial outputs of  both males and females. The same technique is also used on our thermal face data acquired using prototype thermal camera (developed under HeliausEUproject) in an indoor lab environment which is then used for generating synthetic 3D face data along with varying yaw face angles and lastly facial depth map is generated.

% \par  A  person’s   face   discloses   important information about  their  affective  state.  Although  there  has  been  extensive research on recognition of facial expressions, the performance of existing approaches is challenged by facial occlusions. Facial occlusions  are  often  treated  as  noise  and  discarded  in  recognition  of  affective  states.  However,  hand  over  face  occlusions can  provide  additional  information  for  recognition  of  some affective  states  such  as  curiosity,  frustration  and  boredom. One of the reasons that this problem has not gained attention is  the  lack  of  naturalistic  occluded  faces  that  contain  handover   face   occlusions   as well as other types of occlusions. Traditional  approaches  for  obtaining  affective  data  are time demanding and expensive, which limits researchers in affectivecomputing  to  work  on  small  datasets.  This  limitation  affectsthe  generalizability  of  models  and  deprives  researchers  fromtaking  advantage  of  recent  advances  in  deep  learning  thathave  shown  great  success  in  many  fields  but  require  largevolumes  of  data.  In  this  paper \cite{nojavanasghari2017hand2face},  we  first  introduce  a  novelframework for synthesizing naturalistic facial occlusions froman  initial  dataset  of  non-occluded  faces  and  separate  imagesof  hands,  reducing  the  costly  process  of  data  collection  andannotation. We then propose a model for facial occlusion typerecognition to differentiate between hand over face occlusionsand other types of occlusions such as scarves, hair, glasses andobjects. Finally, we present a model to localize hand over faceocclusions  and  identify  the  occluded  regions  of  the  face.

% \par Reduced training sets are major problems typically found on the task of offline signature verification. To increase the number of samples, the use of synthetic signatures can be taken into account. In this work \cite{melo2019deep}, a new method for the generation ofsynthetic  offline  signatures  by  using  dynamic  and  static  (real)  ones  is  presented.  The  synthesis  is  here  faced  under  theperspective of supervised training: the learning model is trained to perform the task of online-to-offline signature conversion. Theapproach is based on a deep convolutional neural network. The main goal is to enlarge offline training dataset in order toimprove  performance  of  the  offline  signature  verification  systems.  For  this  purpose,  a  machine-oriented  evaluation  on  theBiosecurID signature dataset is carried out. The use of synthetic samples (in the training phase) generated with the proposedmethod  on  a  state-of-the-art  classification  system  exhibits  performance  similar  to  those  obtained  using  real  signatures;moreover, the combination of real and synthetic signatures in the training set is also able to show improvements of the equal error rate.

% \par Restoration of a 3D face from the mesh image is highly demanded in computer vision applications. 3D face restoration is a challenging task due to the variation of expression, poses, intrinsic geometries, and textures. The proposed technique consists of two main components, namely face restoration and recognition. A novel three‐dimensional (3D) landmark‐based face restoration method is proposed \cite{sharma20213d}. 3D facial landmarks are used in the face recognition technique. It uses the principle of reflection and mid‐face plane for the restoration of facial landmarks. By using the restored 3D face,a deep learning‐based face recognition system is developed. It utilizes the concept of deep features from variational autoencoders. Further, these deep feature embeddings are trained using triplet loss training to increase the distance between embeddings of different persons and decreasing the distance between embeddings of the same person. These trained embeddings are used in support vector machine for prediction. The proposed framework is compared with recently developed face recognition techniques in terms of computational time. The proposed technique is able to recognize the person's face with better accuracy than the existing methods. Further, ablation studies are conducted to test the robustness of the proposed technique.

% \par Traditional3D face models learn a latent representation of faces using linear subspaces from limited scans of a single database. The main roadblock of building a large-scale face model from diverse3D databases lies in the lack ofdense correspondence among raw scans.  To address these problems, this paper \cite{liu20193d} proposes an innovative framework to jointly learn a nonlinear face model from a diverse set of raw3D scan databases and establish dense point-to-point correspondence among their scans. Specifically, by treating input  scans  as  unorganized point clouds,  we  explore  the use of PointNet architectures for converting point clouds to  identity and expression feature representations, from which the decoder networks recover their 3D face shapes. Further, we propose a weakly supervised learning approach that does not require correspondence label for the scans. We demonstrate  the  superior  dense  correspondence and representation  power  of  our  proposed  method, and  its contribution to single-image3D face reconstruction.  By using a mixture of synthetic and real3D scan data with an effective weakly-supervised learning-based approach, our network can preserve high-frequency details of3D scans.

% \par Recent  advances  in  deep  learning  methods  have  increased  the  performance  of  face  detection  and  recognition systems. The accuracy of these models relies on  the  range  of  variation  provided  in  the  training  data. Creating  a  dataset  that  represents  all  variations  of  real-world faces is not feasible as the control over the quality of   the   data   decreases   with   the   size   of   the   dataset.   Repeatability  of  data  is  another  challenge  as  it  is  not  possible   to   exactly   recreate   ‘real-world’   acquisition   conditions  outside  of  the  laboratory.  In  this  work \cite{basak2020methodology},  we  explore a framework to synthetically generate facial data to  be  used  as  part  of  a  toolchain  to  generate  very  large  facial  datasets  with  a  high  degree  of  control  over  facial  and environmental variations. Such large datasets can be used  for  improved,  targeted  training  of  deep  neural  networks. In particular, we make use of a 3D morphable face model for the rendering of multiple 2D images across a dataset of 100 synthetic identities, providing full control over  image  variations  such  as  pose,  illumination,  and  background. 

% \par Matching  people  in  different cameras,  commonly referred  to  as  person re-identification,  is  a  challenging  task. The   challenges   come   from   the   drastic   appearance   variation across  different  camera  views  caused  by  changes  in  pose,  lighting  condition,  occlusion,  background,  and  so  on.  Instead   of matching  images  in  the  original  feature  space,  many  existing methods learn  distance  metrics  or  feature  transformations  to improve the matching accuracy. For example, data from different camera  views  can  be  projected  onto  their  common  space  to mitigate  the  feature  gap  caused  by  view  discrepancy.  However, a  single-step  mapping may  not  be  sufficient  to  close  this  gap  as the view difference can be significant between different cameras. To  overcome  this  limitation,  we  propose \cite{an2017multi}  a  multi-level  common space  learning  framework,  which  can  gradually  minimize  the data discrepancy between different views in an iterative manner. At  each  intermediate  level,  synthetic  data  are  generated  using the  automatically  discovered  grouping  information,  and  these synthetic data can  be viewed as a transitional state between the original  camera  views.  The  matching  is  performed  by  mapping the probe and gallery onto their common space in multiple steps. We  evaluate  the  proposed  method  on  two  widely  used  person re-identification  data  sets.  The  results  show  that  the  proposed multi-level scheme significantly outperforms single-level mapping.In  addition,  competitive  results  are  achieved  as  compared  with over  20 state-of-the-art  techniques.

% \par Face verification between ID photos and life photos (FV-BIL) is gaining traction with the rapid development of the Internet. However, ID photos provided by the Chinese ad-ministration center are often corrupted with wavy lines to prevent misuse, which poses great difficulty to accurate FV-BIL. Therefore, this paper \cite{zhang2016multi} tries to improve the verification performance by studying a new problem,i.e.blind face in-painting, where we aim at restoring clean face images from the corrupted ID photos. The term blind indicates that the locations of corruptions are not known in advance. We formulate blind face inpainting as a joint detection and reconstruction problem. A multi-task ConvNet is accordingly developed to facilitate end to end network training for accurate and fast inpainting. The ConvNet is used to(i) regress the residual values between the clean/corrupted ID photo pairs and (ii) predict the positions of residual regions. Moreover, to achieve better inpainting results, we employ a skip connection to fuse information in the interme-diate layer. To enable training of our ConvNet, we collect a dataset of synthetic clean/corrupted ID photo pairs with 500 thousand samples from around 10 thousand individuals. Experiments demonstrate that our multi-task ConvNetachieves superior performance in terms of reconstructionerrors, convergence speed and verification accuracy.

% \par Biometrics fingerprint matching has been done witha heavily hand-tuned and designed process of classical computervision  techniques  for  several  decades.  This  approach  has  ledto  accurate  solutions  for  solving  crimes  today  and,  as  such,little  effort  has  been  devoted  to  using  deep  learning  in  this domain.  Given  that  convolutional  neural  networks  have  showndominance for most other image-based problems, we re-evaluatetheir potential for improving the fingerprint matching process. By leveraging synthetic data generators, we show \cite{raff2018neural} that one can train a neural fingerprint enhancer to improve matching accuracy on real  fingerprint  images.  Our  approach  is  both  simple  in  design and  for  potential  deployment  and  adoption  in  real  world  use. 

% \par The  human  eye contains valuable  information  about an individual’s identity  and  health.  Therefore, segmenting  the  eye into  distinct regions  is  an  essential  step  towards  gathering  this useful information  precisely. The main challenges in segmenting the human eye include low light conditions, reflections on the eye, variations in the eyelid, and head positions that make an eye image hard to segment. For this reason, there is a need for deep neural  networks,  which  are  preferred  due  to  their  success  in  segmentation  problems. However,  deep  neural networks  need  a large  amount  of manually  annotated  data  to  be  trained.  Manual annotation is  a  labor-intensive task, and to tackle this problem, we used data augmentation methods to improve synthetic data. In this paper \cite{oz2021use}, we detail the exploration of the scenario,which, with limited data, whether performance can be enhanced using similar context  data  with  image  augmentation  methods.  Our  training  and  test  set  consists  of  3D  synthetic  eye  images generated from the UnityEyes application and manually annotated real-life eye images, respectively. We examined the  effect  of  using  synthetic  eye  images  with  the  Deeplabv3+  network  in  different  conditions  using  image augmentation  methods  on  the  synthetic  data. According  to  our  experiments,  the  network  trained  with  processed synthetic images beside real-life images produced better mIoU results than the network, which only trained with real-life  images  in  the  Base  dataset.  We  also observed  mIoU increase  in  the test  set we  created  from  MICHE  II competition images.

% \par Reconstructing the detailed geometric structure of a face from a given image is a key to many computer vision and graphics applications, such as motion capture and reenactment. The reconstruction task is challenging as human faces vary extensively when considering expressions, poses, textures, and intrinsic geometries. While many approaches
% tackle this complexity by using additional data to reconstruct the face of a single subject, extracting facial surface from a single image remains a difficult problem. As a result, single-image based methods can usually provide only a rough estimate of the facial geometry. In contrast, we  \cite{richardson2017learning} propose to leverage the power of convolutional neural networks to produce a highly detailed face reconstruction from a single image. For this purpose, we introduce an end-to-end
% CNN framework which derives the shape in a coarse-to-fine fashion. The proposed architecture is composed of two main blocks, a network that recovers the coarse facial geometry (CoarseNet), followed by a CNN that refines the facial features of that geometry (FineNet). The proposed networks are connected by a novel layer which renders a depth image given a mesh in 3D. Unlike object recognition and detection problems, there are no suitable datasets for training CNNs
% to perform face geometry reconstruction. Therefore, our training regime begins with a supervised phase, based on synthetic images, followed by an unsupervised phase that
% uses only unconstrained facial images. The accuracy and robustness of the proposed model is demonstrated by both qualitative and quantitative evaluation tests.

% \par Biometrics has become ubiquitous and spurred
% common use in many authentication mechanisms. Keystroke dynamics is a form of behavioral biometrics that can be used for user authentication while actively working at a terminal. The proposed mechanisms involve digraph, trigraph and n-graph analysis as separate solutions or suggest a fusion mechanism
% with certain limitations. However, deep learning can be used as a unifying machine learning technique that consolidates the power of all different features since it has shown tremendous
% results in image recognition and natural language processing. In this paper \cite{cceker2017sensitivity}, we investigate the applicability of deep learning on three different datasets by using convolutional neural networks
% and Gaussian data augmentation technique. We achieve 10\% higher accuracy and 7.3\% lower equal error rate (EER) than existing methods. Also, our sensitivity analysis indicates that the
% convolution operation and the fully-connected layer are the most prominent factors that affect the accuracy and the convergence rate of a network trained with keystroke data.

% \par In this paper \cite{ferrer2014static} we propose a new method for generating synthetic handwritten signature images for biometric applications. The procedures we introduce imitate the mechanism of motor equivalence which divides human handwriting into two steps: the working
% out of an effector independent action plan and its execution via the corresponding neuromuscular path. The action plan is represented as a trajectory on a spatial grid. This contains both the signature text and its flourish, if there is one. The neuromuscular path is simulated by applying a kinematic Kaiser filter to the trajectory plan. The length of the filter depends on the pen speed which is generated using a scalar version of the sigma lognormal model. An ink deposition model, applied pixel by pixel to the pen trajectory, provides realistic static signature images. The lexical and morphological properties of the synthesized signatures as well as the range of the synthesis parameters have been estimated from real databases of real signatures such as the MCYT Off-line and the
% GPDS960GraySignature corpuses. The performance experiments show that by tuning only four parameters it is possible to generate synthetic identities with different stability and forgers with different skills. Therefore it is possible to create datasets of synthetic signatures with a performance similar to databases of real signatures. Moreover, we can customize the created dataset to produce skilled forgeries or simple forgeries which are easier to detect, depending on what the researcher needs. Perceptual evaluation gives an average confusion of 44.06 percent between real and synthetic signatures which shows the realism of the synthetic ones. The utility of the synthesized signatures is demonstrated by studying the influence of the pen type and number of users on an automatic signature verifier.

% \par Recently, counting the number of people for crowd scenes is a hot topic because of its widespread applications (e.g. video surveillance, public security). It is a difficult task
% in the wild: changeable environment, large-range number of people cause the current methods can not work well. In addition, due to the scarce data, many methods suffer from over-fitting to a different extent. To remedy the above two
% problems, firstly, we \cite{wang2019learning} develop a data collector and labeler, which can generate the synthetic crowd scenes and simultaneously annotate them without any manpower. Based on it, we build a large-scale, diverse synthetic dataset. Secondly, we propose two schemes that exploit the synthetic data to boost the performance of crowd counting in the wild: 1) pretrain a crowd counter on the synthetic data, then finetune it using the real data, which significantly prompts the model’s performance on real data; 2) propose a crowd counting method via domain adaptation, which can free humans from heavy data annotations. Extensive experiments show that the first method achieves the state-of-the-art performance on four real datasets, and the second outperforms
% our baselines.

% \par Human-centered data collection is typically costly and implicates issues of privacy. Various solutions have been proposed in the literature to reduce this cost, such as crowd-sourced data collection, or the use of semisupervised
% algorithms. However, semisupervised algorithms require a source of unlabeled data, and crowd-sourcing methods require numbers of active participants. An alternative passive data collection modality is fingerprint-based localization. Such methods use received signal strength or channel state information in wireless sensor networks to localize users in
% indoor/outdoor environments. In this letter \cite{nabati2020using}, we introduce a novel approach to reduce training data collection costs in fingerprint-based localization by using synthetic data. Generative adversarial networks (GANs) are used to learn the
% distribution of a limited sample of collected data and, following this, to produce synthetic data that can be used to augment the real collected data in order to increase overall positioning accuracy. Experimental results on a benchmark dataset show that by applying the proposed method and using a combination of 10\% collected data and 90\% synthetic data, we can obtain essentially similar positioning accuracy to that which would be obtained by using the full set of collected data. This means that by employing GAN-generated synthetic data, we can use 90\% less real data, thereby reducing
% data-collection costs while achieving acceptable accuracy.

% \par Deep learning has catalysed progress in tasks such as face recognition and analysis, leading to a quick integration of technological solutions in multiple layers of our society. While such systems have proven to be accurate by standard evaluation metrics and benchmarks, a surge of work has recently exposed the demographic bias that such algorithms exhibit–highlighting that accuracy does not entail fairness. Clearly, deploying biased systems under real-world settings can have grave consequences for affected populations. Indeed, learning methods are prone to inheriting, or even amplifying the bias present in a training set, manifested by uneven representation across demographic groups. In facial datasets, this particularly relates to attributes such as skin tone, gender, and age. In this work, we address the problem of mitigating bias in facial datasets by data augmentation. We \cite{georgopoulos2021mitigating} propose a multi-attribute framework that can successfully transfer complex, multi-scale facial patterns even if these belong to underrepresented groups in the training set. This is achieved by relaxing the rigid dependence on a single attribute label, and further introducing a tensor-based mixing structure that captures multiplicative interactions between attributes in a multilinear fashion. We evaluate our method with an extensive set of qualitative and quantitative experiments on several datasets, with rigorous comparisons to state-of-the-art methods. We find that the proposed framework can successfully mitigate dataset bias, as evinced by extensive evaluations on established diversity metrics, while significantly improving fairness metrics such as equality of opportunity.

==> content/07-futureApplications.tex <==
\section{Future Applications}
\label{sec:future}
So far, synthetic data has been abundantly utilized by several studies in human analysis. However, several fields of research that use synthetic data such as active learning \cite{gonsior2021imital, budd2021survey}, knowledge distillation \cite{binici2022preventing} and source-free domain adaptation \cite{li2020model, kurmi2021domain} are relatively unexplored for human analysis. In the future, human analysis models can exploit synthetic data for these challenging scenarios.
